EGBTER: Capturing degree distribution, clustering coefficients, and community structure in a single random graph model

Random graph models are important constructs for data analytic applications as well as pure mathematical developments, as they provide capabilities for network synthesis and principled analysis. Several models have been developed with the aim of faithfully preserving important graph metrics and substructures. With the goal of capturing degree distribution, clustering coefficient, and communities in a single random graph model, we propose a new model to address shortcomings in a progression of network modeling capabilities. The Block Two-Level Erd{\H{o}}s-R{\'e}nyi (BTER) model of Seshadhri et al., designed to allow prescription of expected degree and clustering coefficient distributions, neglects community modeling, while the Generalized BTER (GBTER) model of Bridges et al., designed to add community modeling capabilities to BTER, struggles to faithfully represent all three characteristics simultaneously. In this work, we fit BTER and two GBTER configurations to several real-world networks and compare the results with that of our new model, the Extended GBTER (EGBTER) model. Our results support that EBGTER adds a community-modeling flexibility to BTER, while retaining a satisfactory level of accuracy in terms of degree and clustering coefficient. Our insights and empirical testing of previous models as well as the new model are novel contributions to the literature.

==> 02-top-matter.tex <==
\title*{EGBTER: Capturing degree distribution, clustering coefficients, and community structure in a single random graph model\thanks{\scriptsize{This manuscript has been authored by UT-Battelle, LLC under Contract No. DE-AC05-00OR22725 with the U.S. Department of Energy. The United States Government retains and the publisher, by accepting the article for publication, acknowledges that the United States Government retains a non-exclusive, paid-up, irrevocable, world-wide license to publish or reproduce the published form of this manuscript, or allow others to do so, for United States Government purposes. The Department of Energy will provide public access to these results of federally sponsored research in accordance with the DOE Public Access Plan (\url{http://energy.gov/downloads/doe-public-access-plan}).}}
}
\titlerunning{EGBTER: Capturing degree dist., clust. coeff., and community structure }
\author{Omar Eldaghar, Robert A. Bridges, and Erik Lundberg}
% \authorrunning{Short Title} 
\institute{Omar Eldaghar 
	    \at Department of Mathematics, Purdue University, West Lafayette, IN, 47907 $|$
	    % \at Department of Mathematics, Florida Atlantic University, Boca Raton, FL 33431  \&
	    % \at Computational Sciences and Engineering Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831 $|$
	    \email{oeldaghar2013@gmail.com}
	    \and Robert A. Bridges \at Computational Sciences and Engineering Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831$|$ \email{bridgesra@ornl.gov} 
		\and Erik Lundberg \at Department of Mathematics, Florida Atlantic University,  Boca Raton, FL 33431 $|$ \email{elunder@fau.edu}
}
\maketitle	

==> 10-abstract.tex <==
\abstract{
Random graph models are important constructs for data analytic applications as well as pure mathematical developments, as they provide capabilities for network synthesis and principled analysis. 
Several models have been developed with the aim of faithfully preserving important graph metrics and substructures. 
With the goal of capturing degree distribution, clustering coefficient, and communities in a single random graph model, we propose a new model (EGBTER) to address shortcomings in a progression of network modeling capabilities.  
The BTER model of Seshadhri et al. 2012, designed to allow prescription of expected degree and clustering coefficient distributions, neglects community modeling, while GBTER of Bridges et al. 2015, designed to add community modeling capabilities to BTER, struggles to faithfully represent all three characteristics simultaneously. 
In this work, we fit BTER and two GBTER configurations to several real-world networks and compare the results with that of the EGBTER model. 
Our results support that EBGTER adds a community-modeling flexibility to BTER, while retaining a satisfactory level of accuracy in terms of degree and clustering coefficient. 
Our insights and empirical testing of previous models as well as the new model are novel contributions to the literature. 
}

% As a baseline, we fit BTER and two GBTER configurations to several real-world networks and compare the results with that of the EGBTER model. This facilitates quantifiable, qualitative, and visual head-to-head analysis.
% Our results confirm that community structure is not well preserved by the BTER model, while clustering coefficient and degree distributions are not simultaneously preserved by GBTER. 
% Overall, EBGTER adds a community-modeling flexibility to BTER, while exhibiting a balanced accuracy in terms of degree, clustering coefficient, and community structure metrics.
% Our insights and empirical testing of previous models as well as the new model are novel contributions to the literature. 


%Our work builds on a progression of random graph models, from (Erd\"{o}s-R\'{e}nyi) modeling edge density, to (Chung-Lu) modeling degree distribution, to 
%Block Two-Level Erd\"{o}s-R\'{e}nyi 
%BTER, of Seshadhri et al., modeling degree and clustering coefficient distributions, to GBTER, of Bridges et al., allowing flexibility for modeling community structure (possibly  in lieu of clustering coefficients) as well as degree distribution.  



% Complex networks, especially those arising from natural representations of real world data, exhibit structural idiosyncrasies,  which are measured and deduced using many heterogeneous graph metrics, e.g., distributions of degrees, clustering coefficients, and motifs as well as measures of size, centrality, and modularity, to name a few. 
% Consequently, a major focus in random graph models has been on identifying those graph metrics that are important in real-world graph representations and developing models that preserve these metrics. \\
% \indent 




% Block Two-Level Erdos-Renyi (BTER) model of Seshadhri et al.
% evaluating efficacy of two previous models  %\cite{seshadhri2012community} 
% and Generalized BTER (GBTER) model of Bridges et al.) %\cite{bridges2016multi}
% with respect to 
% Specifically, evaluate the modeling capabilities 
% providing detailed novel analysis of the BTER model of Seshadhri et al.'s and GBTER model or Bridges et al. on many real-world networks. 

% introduces a new random graph model for networks with undirected edges. We build on two previous models, the Block Two-Level Erdos-Renyi (BTER) model of Seshadhri et al. \cite{seshadhri2012community} and the Generalized BTER (GBTER) model of Bridges et al. \cite{bridges2016multi}. Previous models for network simulation fail to model the inherent community structure of a network, degree distribution and clustering coefficient per degree distribution simultaneously. To our knowledge, our new model is the first attempt to do so. We provide metrics for each of those quantities and show that while our model does not performs the best in all three major categories, it does not completely overlook one metric in favor of the other two or miss a metric entirely. We also briefly discuss future work that would make this model scaleable.





